Evaluation of User Perception on Biometric Fingerprint System

Biometric systems involve security assurance to make our system highly secured and robust. Nowadays, biometric technology has been fixed into new systems with the aim of enforcing strong privacy and security. Several innovative system have been introduced, and most of them have biometrics installed to protect military bases, banking machines, and other sophisticated systems, such as online tracking systems. Businesses can now focus on their core functions and feel confident about their data security. Despite the benefits and enhancements in security that biometrics offer, there are also some vulnerabilities. This study aimed to investigate the biometric vulnerabilities in a healthcare facility and propose possible countermeasures for biometric system vulnerabilities.

==> cheat-sheet1.tex <==


\section{This is from cheat-sheet}


Some characters:

\#
\$
\%
% percent sign is used for commenting
\&
\{
\}
\_
$|$ or $\mid$
$<$
$>$
$\backslash$

$$\sum_{i=1}^\infty \frac{1}{2^{i+3}} = 1$$

\section{A section title}
Test test test test test test test test test test test test
Test Test Test Test Test Test Test Test Test Test Test Test 

\subsection{A subsection title}
Test Test Test Test Test Test Test Test Test Test Test Test 
Test Test Test Test Test Test Test Test Test Test Test Test 
This is how to cite \cite{Farhadi-12}. 

\subsubsection{A sub sub section title}
Test Test Test Test Test Test Test Test Test Test Test Test 
Test Test Test Test Test Test Test Test Test Test Test Test 


Unordered list:

\begin{itemize}
\item This is one item.
\item This is another.
\end{itemize}

Ordered list:

\begin{enumerate}
\item This is the first item.
\item This is the second.
\end{enumerate}

{\bf Bold, italics and underlining}

Some of the \textbf{greatest} 
discoveries in \underline{science} 
were made by \textbf{\textit{accident}}.

Line breaks 
are straightforward,\\
a double backslash does the trick

``This is a double quote.'' and `Here is a single quote.'

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.3\linewidth]{f1.jpg}
  \caption{Pattern of Vertebrate Embryo in Zebrafish}
  \label{f1}
\end{figure}

See Figure \ref{f1} for details.

See Table \ref{table1} for details.

\begin{table*}
  \caption{Table caption}
  \label{table1}
  \setlength\tabcolsep{3pt}
  \begin{tabular}{|p{4cm}|p{2cm}|p{2.5cm}|}
    \hline
    column title & column title &column title \\
    \hline
    One&Two&Three\\
    \hline
    One&Two&Three\\
    \hline
  \end{tabular}
\end{table*}

Math expressions are separate from text in LATEX. To enter a math environment in the middle of text, use
the dollar sign \$, for example $F = ma$ produces F = ma. Everything between the two dollar signs \$ will be
considered math formula.

To type a math expression that is on its own line and centered, use \$\$:

The following is an important equation:
$$E = mc^2$$

In a document there are different types of \textbf{commands} 
that define the way the elements are displayed. This 
commands may insert special elements: $\alpha \beta \Gamma$







==> sn-bibliography <==
%% Journal article
@article{bib1,
  author		= "Campbell, S. L. and Gear, C. W.",
  title			= "The index of general nonlinear {D}{A}{E}{S}",
  journal		= "Numer. {M}ath.",
  volume		= "72",
  number		= "2",
  pages			= "173--196",
  year			= "1995"
}

%% Journal article with DOI
@article{bib2,
  author		= "Slifka, M. K. and Whitton, J. L.",
  title			= "Clinical implications of dysregulated cytokine production",
  journal		= "J. {M}ol. {M}ed.",
  volume		= "78",
  pages			= "74--80",
  year			= "2000",
  doi			= "10.1007/s001090000086"
}

%% Journal article
@article{bib3,
  author		= "Hamburger, C.",
  title			= "Quasimonotonicity, regularity and duality for nonlinear systems of 
					partial differential equations",
  journal		= "Ann. Mat. Pura. Appl.",
  volume		= "169",
  number		= "2",
  pages			= "321--354",
  year			= "1995"
}

%% book, authored
@book{bib4,
  author		= "Geddes, K. O. and Czapor, S. R. and Labahn, G.",
  title			= "Algorithms for {C}omputer {A}lgebra",
  address		= "Boston",
  publisher		= "Kluwer",
  year			= "1992"
}

%% Item 8. Book, chapter
@incollection{bib5,
  author		= "Broy, M.",
  title			= "Software engineering---from auxiliary to key technologies",
  editor		= "Broy, M. and Denert, E.",
  booktitle		= "Software Pioneers",
  pages			= "10--13",
  address		= "New {Y}ork",
  publisher		= "Springer",
  year			= "1992"
}

%% Book, edited
@book{bib6,
  editor		= "Seymour, R. S.",
  title			= "Conductive {P}olymers",
  address		= "New {Y}ork",
  publisher		= "Plenum",
  year			= "1981"
}

%% Chapter in a book in a series with volume titles
@inproceedings{bib7,
  author		= "Smith, S. E.",
  title			= "Neuromuscular blocking drugs in man",
  editor		= "Zaimis, E.",
  volume		= "42",
  booktitle		= "Neuromuscular junction. {H}andbook of experimental pharmacology",
  pages			= "593--660",
  address		= "Heidelberg",
  publisher		= "Springer",
  year			= "1976"
}

%% Paper presented at a conference
@misc{bib8,
  author		= "Chung, S. T. and Morris, R. L.",
  title			= "Isolation and characterization of plasmid deoxyribonucleic acid from 
					Streptomyces fradiae",
  year			= "1978",
  note			= "Paper presented at the 3rd international symposium on the genetics 
					of industrial microorganisms, University of {W}isconsin, {M}adison, 
					4--9 June 1978"
}

%% Data citation example
@misc{bib9,
  author		= "Hao, Z. and AghaKouchak, A. and Nakhjiri, N. and Farahmand, A.",
  title			= "Global integrated drought monitoring and prediction system (GIDMaPS) data sets", 
  year			= "2014",
  note			= "figshare \url{https://doi.org/10.6084/m9.figshare.853801}"
}

%% Preprint citation example
@misc{bib10, 
  author		= "Babichev, S. A. and Ries, J. and Lvovsky, A. I.",
  title			= "Quantum scissors: teleportation of single-mode optical states by means 
					of a nonlocal single photon", 
  year			= "2002",
  note			= "Preprint at \url{https://arxiv.org/abs/quant-ph/0208066v1}"
}

@article{bib11,
  author		= "Beneke, M. and Buchalla, G. and Dunietz, I.",
  title			= "Mixing induced {CP} asymmetries in inclusive {B} decays",
  journal		= "Phys. {L}ett.",
  volume		= "B393",
  year			= "1997",
  pages			= "132-142",
  archivePrefix		= "arXiv",
  eprint		= "0707.3168",
  primaryClass		= "gr-gc"
}

@softmisc{bib12,
  author		= "Stahl, B.",
  title			= "deep{SIP}: deep learning of {S}upernova {I}a {P}arameters",
  version		= "0.42",
  keywords		= "Software",
  howpublished		= "Astrophysics {S}ource {C}ode {L}ibrary",
  year			= "2020",
  month			= "Jun",
  eid			= "ascl:2006.023",
  pages			= "ascl:2006.023",
  archivePrefix		= "ascl",
  eprint		= "2006.023",
  adsurl		= "{https://ui.adsabs.harvard.edu/abs/2020ascl.soft06023S}",
  adsnote		= "Provided by the SAO/NASA Astrophysics Data System"
}

%%============================================================================%%
%% while using chicago reference style, both abbreviated and expanded form of %%
%% author name format is acceptable. Refer below example for expanded form    %%
%%============================================================================%%

%%  author		= "{Cameron, Deborah}", - single author
%%  author		= "{Saito, Yukio} and {Hyuga, Hiroyuki}", - double author 

%%======================================%%
%% Example for author names with suffix %%
%%======================================%%

%%  author		= "{Price, R. A. Jr} and {Curry, N. {III}} and McCann, K. E. and 
%%					Fielding, J. L. and {Abercrombie, E. Jr}",


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


